Ruledger: Ensuring Execution Integrity in Trigger-Action IoT Platforms

Smart home IoT systems utilize trigger-action platforms, e.g., IFTTT, to manage devices from various vendors. However, they may be abused by triggering malicious rule execution with forged IoT devices or events violating the execution integrity and the intentions of the users. To address this issue, we propose a ledger based IoT platform called Ruledger, which ensures the correct execution of rules by verifying the authenticity of the corresponding information. Ruledger utilizes smart contracts to enforce verifying the information associated with rule executions, e.g., the user and configuration information from users, device events, and triggers in the trigger-action platforms. In particular, we develop three algorithms to enable ledger-wallet based applications for Ruledger and guarantee that the records used for verification are stateful and correct. Thus, the execution integrity of rules is ensured even if devices and platforms in the smart home systems are compromised. We prototype Ruledger in a real IoT platform, i.e., IFTTT, and evaluate the performance with various settings. The experimental results demonstrate Ruledger incurs an average of 12.53% delay, which is acceptable for smart home systems.

==> sections/6-evaluation.tex <==
\section{Implementation And Evaluation}
\red{\textbf{REMOVE this section.}}
% In this section, we evaluate the performance of our \middlewareFull . We first describe how we setup the experiment, then present the test goals and results from two aspects, overhead and throughput. Specifically, we evaluate the overheads of the \middleware and its components, and compare the overall overhead with SmartThings baseline system.

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{table}[h]
\centering
\caption{Deployment Environments} \label{tbl:config}
\begin{tabular}{m{0.12\textwidth}<{\centering} m{0.13\textwidth}<{\centering} m{0.16\textwidth}<{\centering}}
    \hline
    \multirow{2}*{Components} & \multicolumn{2}{c}{Deployment Environment} \\
    \cline{2-3} 
    ~ & Local Deployment & Cloud Deployment   \\
    \hline
    Blockchain &
    \tabincell{l}{Intel NUC8BEH\\CPU: 7-8559U\\Memory: 32G DDR4} &
    \multirow{4}*{\tabincell{l}{Huawei Cloud Server\\ CPU: Intel(R) Xeon(R)\\ Gold 6161, 4 cores,\\2.20GHz Memory: 8GB \\ OS: Ubuntu 16.04 64bit}} \\
    \cline{1-2}
    Task Agent &
    \multirow{2}*{\tabincell{l}{Raspberry Pi 4}} & \\
    \cline{1-1}
    Execution Agent &  & \\
    \cline{1-2}
    Device Simulators &
    \tabincell{l}{Raspberry Pi 3} & \\
    \hline
\end{tabular}
% \footnotesize{}\\
\end{table}

\subsection{Experimental Setup}

We evaluate our \middleware under both local deployment and cloud deployment, which deploy environments are shown in Table \ref{tbl:config}. Two metrics need to be concerned to evaluate the performance of our system, the overhead of rule execution and the throughput. For the former, since the \middleware adds an additional part to the traditional architecture of IoT device collaborations, we only evaluate that the additional overhead introduced by the \middleware and time-overhead required by each components of it are acceptable. For the latter, the evaluation of the throughput is used to demonstrate the scalability of our \middleware. 

Since the execution agent and the task agent in the \middleware can be horizontal scaled, we test an unit \middleware, which includes an execution agent of the trigger IoT service, an execution agent of the action IoT service, a task agent of one user and a ledger-based IoT framework, to evaluate the overall overhead that is introduced by our \middleware, and test each component separately to evaluate the scalability of the \middleware. Moreover, we compare the time-overhead of the \middleware with SmartThings baseline system in the cloud deployment environment, since the SmartThings baseline system does not support local deployment. The evaluations are based on rules with one trigger event and one action task since this type of the rules are most commonly used on the trigger-action platforms.

% \textbf{environment setup}
% We deploy our middleware prototype both on cloud servers and local devices as Table \ref{tbl:config} shows and evaluate their performance. The cloud servers run 64-bit Ubuntu 16.04 with 2.2 GHZ quad core processor. The local devices are a Intel NUC8BEH micro server running 64-bit Ubuntu 16.04 with i7-8559 CPU and 32G memory, a Raspberry 4 and a Raspberry 3. As we discussed in Section \ref{sec: design}, the smart contracts can serve as server programs once they are deployed on the blockchain platform. We register the public keys of the task agent and the execution agents while deploying the contracts. Then each execution agent gets notification to retrieve an executory device script and starts to run, after any IoT rule is configured through the task agent. Note that the number of these agents depends on the amount of users, collaborative IoT services and execution requests. However, the performance of multi-users scenario depends much more on the implementation detail, especially of the agents. Therefore, we only test the minimum system unit that consists of one task agent and two execution agents, to evaluate the scenario composed by one user and two IoT services.

% \textbf{Ground-truth}
% The performance of the system unit depends on the complexity of user's IoT rule, which is up to composition of the trigger condition and the number of actions in one IoT rule. Since most of the rules on the trigger-action platforms contain one trigger condition and one action service but may trigger several action tasks, we only need to construct IoT rules based on the number of action tasks rather than whole content of the rules. In addition, the action tasks on the trigger-action platform can be divided into three categories, main actor, standby actor and notifying actor. Besides, a trigger-action rule executes one action task for each category in most of the case. Thus, we range the number of action tasks from one to three in one rule to construct the IoT rules. Moreover, the storage overhead of the IoT rule depends not only on the number of action tasks, but also the expression of the device scripts to measure the system performance. Since the majority of the IoT cloud services supports Restful cloud device APIs or Restful device handler, the difference of storage overhead between device scripts is negligible. In conclusion, IoT rules with various number of action tasks and one trigger condition can be constructed for evaluating the performance of our system unit.

% \textbf{Data configuration}
% We configure one IoT rule on the distributed ledger for micro-benchmarks and 200 IoT rules for macro-benchmarks, using the task agent deployed in advance. In order to evaluate the performance of executing the IoT rule, we various the action tasks in one IoT rule from one to three in micro-benchmarks. However, to make a better performance evaluation of the system unit in macro-benchmarks, we simplify the 200 IoT rules with only one action task in each of them. Additionally, since t
he consortium distributed ledger is composed by nodes of all the collaborative IoT platforms, and there is at least two IoT platforms including IFTTT in the home-based scenario of one user, we range number of the nodes from 4 to 10, increasing by 2 nodes for each group of tests, to to evaluate the time performance of rule execution.



\subsection{Overheads of \ourwork}

In this part, we evaluate the overheads introduced by our \middleware and its components separately, and compare the overall execution-time overhead with Smartthings baseline system, which uses the traditional IoT architecture for device collaboration, to evaluate whether the overheads required by the \middleware is acceptable in order to protect the integrity of the rule execution.

\textbf{1. Overheads of the Components}

we first quantify the execution-time overheads of two \middleware components, which are the execution agent and the ledger service, under varies amounts of concurrent requests that executes 1, 10 and 100 different rules separately. The amount of concurrent requests to an execution agent ranges from 10 to 100, and the amount of the execution agent is scaled horizontally from 1 to 20 to reach the upper limit for the number of concurrent requests on the IFTTT.

\textit{\textbf{Execution Agent}}
The execution agent requires an additional time-overhead to submit an unverified trigger event to the ledger service and receive the consensus result of verifying the event’s integrity.

The Execution Agent of each IoT service can be deployed both on the cloud server and the local device, such as an wearable device or a smart gateway. When deployed on the cloud, the execution agent can be scaled horizontally to handle more concurrent requests. Therefore, we study the average time-overhead of executing 1, 10 and 100 different rules by varying the concurrency and the amount of the execution agent. The experiment result is shown in Figure \ref{fig: cloud_ea}.

\begin{figure}[h]
\centering
\includegraphics[scale=0.16]{figrues/ear.eps}
% \captionsetup{justification=centering}
\caption{The average time-overhead of executing 1, 10 and 100 different rules with varies amount of concurrent requests and varies amount of the execution agent.}
\label{fig: cloud_ea}
\end{figure}

In common cases, only one execution agent is required for each IoT service when deployed locally, and high-concurrecy of rule execution is not needed in the local environment. Thus, we test the average time-overhead of the execution agent when executing 1, 10 and 100 different rules, with a load of 10 concurrent requests. The results are shown in Table \ref{tbl: local_ea}

% \begin{table}[]
% \centering
% \caption{The average time-overhead of the execution agent in local deployment environments} \label{tbl: local_ea}
% \begin{tabular}{c|c|c|c}
% \hline
% \begin{tabular}[c]{@{}c@{}}Number of different rules \\ that are executed concurrently\end{tabular} & 1 rules & 10 rules & 100 rules \\ \hline
% The average time-overhead (ms)                                                                      &   &    &     \\ \hline
% \end{tabular}
% \end{table}



The above test results demonstrate that the time-overhead of the execution agent is acceptable and has the potential to expand horizontally, in order to protect the device execution and verify the integrity of the execution. Besides, it can adapt to both local and cloud deployment for different use cases.


\textit{\textbf{Ledger Service}}
The ledger service needs an additional time-overhead to retrieve a trigger event and submit a corresponding action task. Specifically, the task submitting process contains the execution time on the ledger-based IoT framework that verifies the preceding event on the smart contract and verifies the integrity of the action task through consensus mechanism.

Since the user’s task agent of the ledger service also supports horizontal scaling for multi-users or for one when it is deployed on the cloud as a web application, we investigate the time-overhead of the ledger service when executing 1, 10 and 100 different rules, by varying the amount of concurrent requests and the number of the task agent, under the cloud deployment environment. The variation trend of the average time-overhead is shown in Figure \ref{fig: cloud_ls}.

\begin{figure}[h]
\centering
\includegraphics[scale=0.16]{figrues/tar.eps}
% \captionsetup{justification=centering}
\caption{The average time-overhead of executing 1, 10 and 100 different rules with varies amount of concurrent requests and varies amount of the ledger service.}
\label{fig: cloud_ls}
\end{figure}

Similarly, the ledger service can be deployed locally in an working area or at the user’s home, where high-concurrency is not required usually. Therefore, we only evaluate the average time-overhead of the ledger service under a load of 50 concurrent requests, when it executes 1, 10 and 100 different rules separately, which results are presented in Table \ref{tbl: local_ls}.

% \begin{table}[]
% \centering
% \caption{The average time-overhead of the ledger service in local deployment environments} \label{tbl: local_ls}
% \begin{tabular}{c|c|c|c}
% \hline
% \begin{tabular}[c]{@{}c@{}}Number of different rules \\ that are executed concurrently\end{tabular} & 1 rules & 10 rules & 100 rules \\ \hline
% The average time-overhead (ms)                                                                      &   &    &     \\ \hline
% \end{tabular}
% \end{table}

The evaluation result of the ledger service shows that the ledger service can ensure the integrity of rule execution at the expense of acceptable overhead and supports horizontal scaling to meet the demand of accessing multi-users. What’s more, the wallet-based service satisfies the following design principles, 1) independent of any user’s trusted nodes, 2) least changes to the current trigger-action platforms.

We further study the time-overhead introduced by the ledger-based IoT framework of the ledger service to evaluate whether the performance of ledger is the bottleneck of our \middleware. Since the ledger takes each rule execution request as a different transaction, we measure the execution time on the ledger-based IoT framework which executes one same rule, by varying the amount of concurrent transactions and the number of ledger nodes. Besides, the consortium blockchain relies on the identity authentication mechanism to protect the integrity of rule execution process instead of the enormous amount of nodes, we conduct this experiment under four common configurations of different numbers of ledger nodes. The result is given as Figure \ref{fig: LIF-time}.

% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.30]{figrues/Test2.png}
% % \captionsetup{justification=centering}
% \caption{The average time-overhead of the ledger-based IoT framework with varies amount of concurrent requests and varies number of the ledger nodes.}
% \label{fig: LIF-time}
% \end{figure}

This experiment result gives the clear conclusion that the ledger-based IoT framework is able to satisfy a single user’s demand under general concurrency. Moreover, the execution time on the ledger-based IoT framework increases at a low speed with the growing number of ledger nodes


\textbf{2. Overheads of the entire \middleware}

We now evaluate the overall time-overhead added by our \middleware by implementing an IoT system based on our \middleware and comparing it with SmartThings baseline system, in which two device simulators are constructed using SmartThings Groovy IDE and connected to IFTTT. It is noting that this IoT system is built by accessing our \middleware to a SmartThings app, meaning that our \middleware can access either to the current IoT system or to a cloud IoT device platform. Besides, the SmartThings baseline system runs on its cloud server, thus, we measure the average execution time of both systems by triggering one rule execution each of the time. The comparison result is demonstrated in Table \ref{tbl: overall}.

% \begin{table}[]
% \centering
% \caption{The comparison of average execution time-overhead with SmartThings baseline system} \label{tbl: overall}
% \begin{tabular}{cc|c}
% \hline
% \multicolumn{2}{c|}{Average execution time (s)}                                                                                                                                           & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Percentage of the \\ additional time-overhead\\ introduced by \textbackslash{} \middleware \end{tabular}} \\ \cline{1-2}
% \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SmartThing\\ baseline system\end{tabular}} & \begin{tabular}[c]{@{}c@{}}IoT system based\\ on \textbackslash{} \middleware \end{tabular} &                                                                                                                                                     \\ \hline
% \multicolumn{1}{c|}{}                                                                     &                                                                                          &                                                                                                                                                     \\ \hline
% \end{tabular}
% \end{table}


\begin{table}[]
\centering
\caption{The comparison of average execution time-overhead with SmartThings baseline system} \label{tbl: overall}
\begin{tabular}{cccc}
\hline
              & SmartThings & \textbackslash{}ourwork & \begin{tabular}[c]{@{}c@{}}Increased Ratio\\ imposed by \textbackslash{}ourwork\end{tabular} \\ \hline
Time Overhead & 1.403 s     & 1.604 s                 & 14.33\%                                                                                      \\ \hline
\end{tabular}
\end{table}


From this comparison result, we can draw the conclusion that the additional time-overhead introduced by our \middleware is acceptable.

Since the ledger service is the main component in our \middleware, we need to further evaluate the percentage of the time-overhead required by the ledger service in the overall time-overhead of our \middleware. 

Since the ledger service is the main component in our \middleware, we need to further evaluate the percentage of the time-overhead required by the ledger service in the overall time-overhead of our \middleware. In this way, we reomve the ledger service from the IoT system based on \middleware and compare its average overall execution time with the original IoT system, with 10, 100 and 1000 rules executed concurrently. The result is shown in Figure \ref{fig: non-ledger}. 

\begin{figure}[h]
\centering
\includegraphics[scale=0.16]{figrues/ledger.eps}
% \captionsetup{justification=centering}
\caption{Comparing the average execution time between the original IoT system and the system without the ledger service.}
\label{fig: non-ledger}
\end{figure}

The results further demonstrate that the ledger service takes a small part of the overall execution time that our \middleware requires.


% We first quantify micro-benchmarks of the minimum system unit to evaluate its performance under home-based scenario with single user. In order to integrate the current trigger-action platform with our system unit, we create the following trigger-action rule on the IFTTT:"\textit{If Maker Event ‘heart rate alert’, then notify the task agent to open the door.}", and link it with the IoT rule on the distributed ledger using identities of trigger and action events. The test results of the overheads are elaborated below.

% \textbf{1.	Time Overhead}
% This experiment evaluates the time overhead of our middleware system, including the time overhead introduced by our system and the running time of each main step for executing a rule. Since our system need extra interactions with the smart contract to protect the rule execution, we should quantify the time performance of our middleware system's processings and influence of the processing steps.

% To study the time overhead introduced by our middleware system, we first present the end-to-end overhead, the time between when an execution agent starts a trigger task and when another execution agent record the action execution event. Take our experiment for example, this overhead is the time between getting a device script of deciding and triggering a heart rate alert event through the smart contract and recording the "unlock door" action. We trigger the execution agent to retrieve the script and measure each test 30 times. The end-to-end time overhead is on average 3.46 s, in which our system only costs 769.36 ms under cloud deployment except for the latency of communication with IFTTT. We also evaluate the time overhead of our system that is deployed on the local devices, and the results are shown in Table \ref{tbl: time overhead}. The time overhead introduced by our system under cloud deployment constitutes 22.2\% of the end-to-end time overhead. In contrast, our system under local deployment requires an 2.05 s (40.1\%) in the end-to-end time overhead. The difference of the time overhead costed by our system is mainly made up of the communication latency among the system components, since these components run on the same cloud server for the former and run on different local devices for the latter.

% \begin{table}[]
% \centering
% \caption{Time overhead introduced by our system for executing a rule}
% \label{tbl: time overhead}
% \begin{tabular}{c|c|c}
% \toprule[1pt]
% deploy Environment                                         & system time overhead & Percentage \\
% \midrule[0.8pt]
% \begin{tabular}[c]{@{}c@{}}cloud\\ deployment\end{tabular} & 769.36 ms          & 22.2\%     \\ \hline
% \begin{tabular}[c]{@{}c@{}}local\\ deployment\end{tabular} & 2050.63 ms         & 40.1\%     \\ 
% \bottomrule[1pt]
% \end{tabular}
% \end{table}

% We then investigate the time overhead of three different types of operations in our system, (1) the execution time of the distributed ledger operations, (2) the time overhead imposed by the components external to the smart contract, (3) the execution time of the devices. Table \ref{tbl: step overhead} shows the running times of these parts of our prototype. Since our key work is to record and verify the preceding events on the smart contract for each IoT task, and protect the integrity of the task, we should quantify the time overhead required for the smart contract processings. The result shows the event recording takes 270.45 ms (48\%) in the overhead of ledger's main processing and the event verification requires 293.08 ms (52\%). It validates that the time performance of the smart contract processing mainly depends on the consensus speed of the distributed ledger, because the event verification step need to validate rule, event and protocol state additionally, in contrast to the processing of event recording. Note that the time overhead imposed by operations of each component should reflects our key work, we compute the running time required by each agent. The results demonstrate the task agent takes the most of the overhead, 563.54 ms (75.9\%), which is reasonable since in our prototype the task agent waits for retrieving the recorded event and verify it after receiving an action task. Moreover, the total execution time of the devices is 26.7 ms and costs only 3.5\% of the system time overhead. This overhead is measured because executing device scripts is one of our protocol steps. All the running times in Table \ref{tbl: step overhead} are measured from the application code. 

% \begin{table}[ht]
% \centering
% \caption{Time overhead of different operations for executing a rule}
% \label{tbl: step overhead}
% \begin{tabular}{c||c|c}
% % \hline
% \toprule[1pt]
% Operation Section              & Running time       & Percentage     \\ \hline \hline
% \textbf{Ledger Processing}     & \textbf{563.54 ms} & \textbf{100\%} \\ \hline
% event record                   & 270.45 ms          & 48\%           \\ \hline
% event verification             & 293.08 ms          & 52\%           \\ \hline
% \textbf{Components Operations} & \textbf{742.67 ms} & \textbf{100\%} \\ \hline
% trigger execution agent        & 30.71 ms           & 4.1\%          \\ \hline
% task agent                     & 563.54 ms          & 75.9\%         \\ \hline
% action execution agent         & 37.59 ms           & 5.1\%          \\ \hline
% \textbf{Device Execution}      & \textbf{26.7 ms}   & \textbf{100\%} \\ \hline
% execute trigger script         & 23.58 ms           & 88.3\%         \\ \hline
% execute action script          & 3.12 ms            & 11.7\%         \\ \hline
% \end{tabular}
% \end{table}

% We now compare the time overhead of our system and SmartThings to validate the performance of our prototype. The base line system is SmartThings which controls two device simulators, a sensor and a lock and expose the device handlers to a third-party application. We implemented this simple application and connect it to the IFTTT. A trigger-action rule on the IFTTT:"if temperature sensor detects temperatures above 30 $^\circ$C, then unlock door." combines the two simulated devices. The communication latency between each testing system and the IFTTT is excluded from the time overhead of trigger service and action service. Figure \ref{fig:smartthings} demonstrate the results of this experiment. Our results show that our system only adds 44.98 ms (16.1\%) to the trigger service and 99.72 ms (42.6\%) to the action service compared to the SmartThings.

% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.25]{figrues/smartthings.pdf}
% % \captionsetup{justification=centering}
% \caption{Comparison of time overhead with SmartThings}
% \label{fig:smartthings}
% \end{figure}

% We further study the influence of the ledger-based IoT framework on the rule execution by removing the smart contract processings from our system. Since our middleware system without the distributed ledger is architecturally equivalent to the general architectures, which connects IoT cloud services or devices through IFTTT, it can help to eliminate the device differences and implementation performance of the agents by comparing our original system with the ledger-less baseline system. In this way, we can draw more precise conclusion on the performance of the ledger-based IoT framework.   \textcolor{blue}{new experiment to be done...}


% \begin{table*}
% \begin{center}

% \caption{Average Running Time of Main steps} \label{tbl:micro-latency}
% \begin{tabular}{|l|r|r|r|r|}
%     \hline
%     \multirow{2}*{Steps} &
%     \multicolumn{2}{c|}{Cloud Deployment} & \multicolumn{2}{c|}{Local Deployment}\\
%     \cline{2-5} & Running Time & Percentage & Running Time & Percentage \\ \hline
%     1 trigger device scripts retrieving & 12.31 ms & 0.356\% & 139.32 ms & 2.725\% \\ \hline
%     2 trigger device execution & 23.58 ms & 0.681\% & 490.96 ms & 9.604\% \\ \hline
%     3 trigger event submitting & 18.41 ms & 0.532\% & 272.64 ms & 5.333\% \\ \hline
%     4 trigger event retrieving & 270.45 ms & 7.815\% & 420.64 ms & 8.228\% \\ \hline
%     5 action task submitting & 293.08 ms & 8.469\% & 499.13 ms & 9.764\% \\ \hline
%     6 action task retrieving & 6.24 ms & 0.18\% & 111.16 ms & 2.174\% \\ \hline
%     7 action device scripts retrieving & 9.11 ms & 0.263\% & 116.78 ms & 2.284\% \\ \hline
%     8 action device execution & 3.12 ms & 0.09\% & 73.36 ms & 1.435\% \\ \hline
%     9 action record submitting & 22.24 ms & 0.643\% & 283.85 ms & 5.552\% \\ \hline
%     end to end latency & \multicolumn{2}{c|}{3.461 s} & \multicolumn{2}{c|}{5.112 s} \\ \hline
% \end{tabular}
% \end{center}
% \end{table*}



% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.21]{figrues/micro_latency_line1.pdf}
% % \captionsetup{justification=centering}
% \caption{Latency of Each Step}
% \label{fig:micro-step}
% \end{figure}


% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.21]{figrues/micro_latency_bar.pdf}
% % \captionsetup{justification=centering}
% \caption{End-to-end Latency}
% \label{fig:micro-e2e}
% \end{figure}


% % \begin{table}
% % \begin{center}

% % \caption{Average Latency of Main steps (milliseconds)} \label{tbl:micro-latency}
% % \begin{tabular}{|c|c|}
% % \hline
% % trigger event submitting & trigger event retrieving \\
% % \hline
% % 145.5 & 345.5\\
% % \hline
% % action task submitting & action task retrieving \\
% % \hline
% % 396.1 & 58.7\\
% % \hline
% % device script retrieving & action record submitting \\
% % \hline
% % 69.4 & 153 \\
% % \hline
% % \multicolumn{2}{|c|}{IFTTT request latency:  2876.5}     \\
% % \hline
% % \multicolumn{2}{|c|}{Total end-to-end latency:  4443.7}     \\
% % \hline

% % \end{tabular}
% % \end{center}
% % \end{table}


% %
% % ===================== keep ? =================================
% \textbf{2.	Storage Overhead}
% In this experiment, we measure the storage overhead required by our ledger-based IoT framework for storing and executing an IoT rule. The experiment goal is to evaluating the cost for the distributed ledger to store verification data, including the trigger event and the IoT rule, and the verification result, namely the valid action task. The results in Table \ref{tbl: storage} shows that each IoT rule on the distributed ledger creates 0.51KB. Besides, the event that we use to substitute DTAP's fine-grained token for each rule only requires 0.19KB. Our ledger-based IoT framework together costs 0.7KB (9.3\%) storage overhead comparing to 7.5KB of DTAP \cite{dtap18}.

% Except for the above storage overhead of our ledger-based IoT framework, the binary file of the smart contract creates 119KB storage overhead on each distributed ledger node. However, the storage size can not describe precisely the total resources that are consumed on the ledger for processing each transaction. Thus, we test the required gas on EVM for recording and verifying the event to evaluate consumption of CPU, memory and storage. The reult shows the transaction of submitting a trigger event requires a total 28783 gas in which execution of the smart contract takes 3799 gas (13.2\%), and the transaction of verifying and recording an action task needs 34737 gas in which execution of the smart contract takes 8985 gas (25.9\%). Comparing to a transaction for money transfer on the ETH that normally costs 21000 gas, our ledger-based IoT framework works with a reasonable storage overhead.

% \begin{table}[ht]
% \centering
% \caption{Comparison of storage overhead with DATP}
% \label{tbl: storage}
% \begin{tabular}{cc|c|c|c}
% \toprule[1pt]
% \multicolumn{2}{c|}{Ours}            & \multicolumn{2}{c|}{DTAP}                    & Percentage             \\
% \midrule[0.8pt]
% \multicolumn{1}{c|}{rule}  & 0.51KB & rule                & \multirow{2}{*}{7.5KB} & \multirow{2}{*}{9.3\%} \\ \cline{1-3}
% \multicolumn{1}{c|}{event} & 0.19KB & rule-specific token &                        &                        \\
% \bottomrule[1pt]
% \end{tabular}
% \end{table}


% \textbf{3.	Transmission Overhead}
% Finally, we evaluate the transmission overhead introduced by our system for executing a rule. This overhead is the result of transmitting trigger events and action tasks from our system. The goal of this experiment is to quantify the transmission cost for protecting integrity of the transmission data and their execution process. The results are presented in Table \ref{tbl: trans}. Four transmission overhead of our key work is given, and their sum is compared to the transmission overhead of DTAP \cite{dtap18}. Our system only requires 2.67KB (36.8\%) comparing to 7.5KB transmission overhead of DTAP's work.
% It is noting that their another difference lie on the variance of transmission overhead with function parameters, which is not shown in the test results. Since we use smart contract to verify execution of the device script, instead of having action service to verify the transmitted device function, tranmission overhead of our system do not vary over function parameters. It also helps to improve expansibility of our system.


% \begin{table}[ht]
% \centering
% \caption{Comparison of transmission overhead with DATP}
% \label{tbl: trans}
% \begin{tabular}{c|c|c|c|c}
% \toprule[1pt]
% \multicolumn{3}{c|}{Ours}                                     & DTAP                             & Percentage              \\
% \midrule[0.8pt]
% submit a trigger event & 0.57KB & \multirow{4}{*}{2.76KB} & \multirow{4}{*}{7.5KB} & \multirow{4}{*}{36.8\%} \\ \cline{1-2}
% retrieve a trigger event & 0.86KB &                         &                                  &                         \\ \cline{1-2}
% submit an action task  & 0.48KB &                         &                                  &                         \\ \cline{1-2}
% retrieve an action task  & 0.85KB &&                                  &                         \\
% \bottomrule[1pt]
% \end{tabular}
% \end{table}


% \textbf{4.	Development Volume}
% We develop the ledger-based IoT framework as two smart contracts for rule management and execution, which are supported by three extra library contracts, and provide two corresponding libraries for both the users and IoT platforms to connect to our ledger based IoT framework. Developers of the IoT platforms only need to authorize execution right of the device APIs to the execution agent, which can be a third-party application or a native application. Similarly, developers of the user's task agent need to implement additional authorization works between both the trigger-action platform and IoT platforms with itself, in order to set off user's trigger-action rule and obtain the device API to wrap the script. Moreover, our ledger-based IoT framework presents a much more elegant approach for rule execution and verification, since the smart contract substitutes a centralized trusted third party and simplify the protocol interaction.
% In conclusion, our middleware system shows a concise protocol implemented by the smart contract and requires little extra develop effort for the external components.

% \textcolor{blue}{New experiment: Our system compatibility with both device cloud platforms and real IoT platforms like SmartThings as IoT connection service Figure \ref{fig:overview}.}

% %
% % ===================== keep ? =================================

\subsection{Throughput}

In this part, we measure the throughput of a unit \middleware as the number of rules executed per seconds, by varying the number of ledger nodes and the amount of concurrent rules, to study the scalability of the \middleware.

Taking the concurrency as abscissa and the number of executed rules per seconds as ordinate, the throughput for a certain number of the ledger nodes is chosen from either of the following situation. First, the first inflection point appears and the cocurrency does not exceed the max concurrency of the IFTTT. Second, the upper limit of the concurrency is reached before the inflection point appears.

% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.35]{figrues/Test5.png}
% % \captionsetup{justification=centering}
% \caption{Throughput of the \middleware with one execution agent to trigger the rule executions}
% \label{fig: throughput}
% \end{figure}

The best result is presented if the number of nodes has almost no significant influence on the throughput, and the throughput keeps stable for a long time under high-concurrency. In this way, we can draw the conclusion that the unit \middleware is scalable and has potential to be deployed in large-scale.

We also investigate the influence that the number of the execution agent has on the throughput, since the \middleware supports horizontal scaling of the execution agent. The result is presented in Table \ref{tbl: through-scaled}.


% \begin{table}[]
% \centering
% \caption{The throughput of \middleware with the execution agent scaled horizontally} \label{tbl: through-scaled}
% \begin{tabular}{c|c|c|c}
% \hline
% \begin{tabular}[c]{@{}c@{}}Number of execution agent\\ to trigger the rule execution\end{tabular}    & 1 & 5 & 10 \\ \hline
% Throughput (requests/sec)                                                                            &   &   &    \\ \hline
% \begin{tabular}[c]{@{}c@{}}corresponding concurrency of\\ the throughput (requests/sec)\end{tabular} &   &   &    \\ \hline
% \end{tabular}
% \end{table}


\begin{table}[]
\centering
\caption{The throughput of \ourwork and \ourwork that removes off the Ledger Service under a load of concurrency around 2000 reqs/s} \label{tbl: through}
\begin{tabular}{ccc}
\hline
                   & \textbackslash{} \ourwork & \begin{tabular}[c]{@{}c@{}}\textbackslash{} \ourwork that removes off\\ the Ledger Service\end{tabular} \\ \hline
Throughput (req/s) & 40.57                   & 43.37                                                                                        \\ \hline
\end{tabular}
\end{table}



\textcolor{red}{updating here...}






% \begin{figure*}[h]
% \centering
% \includegraphics[scale=0.52]{figrues/macro_through.pdf}
% % \captionsetup{justification=centering}
% \caption{System Throughput}
% \label{fig:macro-throughput}
% \end{figure*}





% We measure the throughput of the minimum system unit as the number of rules executed per seconds. We test the system throughput with different numbers of blockchain nodes. For each group of tests, the number of total requests varies from 2000 to 10000 with the concurrency ranges from 383 requests per seconds to 954 requests per seconds. The result is shown in Table \ref{fig:macro-throughput}.

% The result shows that our system throughput remains a stable level about 35 requests per seconds, even under a total 10000 requests with concurrency more than 900 requests per seconds. Moreover, during the tests, the success rate always keeps more than 95\%. The reason why increasing the number of blockchain nodes has no influence on our system should be that the wallet-based distributed agents helps to release the processing burden of the blockchain, and the performance of our system is able to support large scale deployment. This test result again shows that a minimum system unit is able to support large amount of user requests with multiple edge devices at user's home.

% We vary the number of configured IoT rules from 50 to 1000 to evaluate the influence it has on system throughput. The Picture \ref{fig:r2la} shows that the amount of IoT rules still has no significant influence on the system latency. It means users are able to configure their IoT rules for home-based scenario at will.



% We measure end-to-end latency and throughput of our secure IoT system to evaluate the performance and scalability under multiple requests of the user.

% \textbf{5.	System Latency}

% We measure the time between the triggering Execution Agent submitting an event record to blockchain, and the time the action Execution Agent submitting an execution record. We use JMeter to conduct tests by sending varied numbers of event requests to trigger the Execution Agent. The time that IFTTT takes to receive event notifications and send action requests is excluded from system latency, in order to eliminate effect of rate limiting that platform like IFTTT brings. The latency of retrieving each user’s device scripts from blockchain by the Execution Agent is measured only once, since we cache the same script in the Execution Agent during tests.

% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.19]{figrues/req2la.pdf}
% % \captionsetup{justification=centering}
% \caption{System Latency with Various Requests}
% \label{fig:req2la}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.19]{figrues/con2la.pdf}
% % \captionsetup{justification=centering}
% \caption{System Latency with Various Concurrency}
% \label{fig:con2la}
% \end{figure}

% Since edge devices of a user in home-based scenario won't be too much, we test the system latency with different numbers of blockchain nodes to evaluate the influence that blockchain consensus brings to our system unit. We varies the total amount of execution requests from 50 to 1000 for each group of test, to evaluate the system's performance under multiple user requests. The Picture \ref{fig:req2la} shows that the system latency is stable with nearly linear request-latency relationship, and changes to the number of blockchain node shows no significant difference on system latency. The system latency is 1.28s for 50 requests and increase to 13.4s for 1000 requests. This result does not tell the variation trend with concurrency of requests, which could indicate the influence that concurrent users have on system latency. The Picture \ref{fig:con2la} shows that our system latency is also stable with nearly linear concurrency-latency relationship, and number of blockchain nodes shows no significant influence on the system latency. However, we find that the number of blockchain nodes shows significant influence when the user requests are all submitted to a same blockchain node during the test, as shown in Picture \ref{fig:an2la}. The success rate keeps higher than 98\% when number of blockchain nodes is less than 8, and remains higher than 92\% for no more than 10 blockchain nodes.

% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.19]{figrues/an2la.pdf}
% % \captionsetup{justification=centering}
% \caption{System Latency with Various Requests to one node}
% \label{fig:an2la}
% \end{figure}

% It first illustrate that our system is able to support large amount of user requests with multiple edge devices at user's home, if the Execution Agent of IoT cloud services choose to communicate with randomly selected blockchain nodes. Moreover, our system still remains a latency that less than 4 seconds under 200 total requests and concurrency more than 70 requests per seconds. It also gives the indication that our system could be scalable under multi-users, considering our design is horizontal scalable with different wallet-based Task Agents executing each user's IoT rules.

% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.21]{figrues/r2la.pdf}
% % \captionsetup{justification=centering}
% \caption{System Latency With Various Numbers of IoT Rules}
% \label{fig:r2la}
% \end{figure}

% To further verify the scalability of our system, we vary the number of configured IoT rules from 50 to 1000 on the blockchain. The Picture \ref{fig:r2la} shows that the amount of IoT rules has almost no significant infuence on the system latency. In conclusion, our IoT system shows low latency with high availability and is enough to support home-based scenario for a user. What's more, it shows a great potential to be deployed in large scale with good scalability.



% \begin{figure*}[h]
% \centering
% \includegraphics[scale=0.52]{figrues/macro_latency.pdf}
% % \captionsetup{justification=centering}
% \caption{System Latency}
% \label{fig:macro-latency}
% \end{figure*}

% Since the amount of each user’s rules is determined by the number of smart devices and functionalities that one owns, we vary the number of concurrent execution rules from 10 to 2000 with 4 fixed chain nodes representing user’s edge devices at home. For each group of tests, the number of rules configured on blockchain is 20 and the concurrent requests trigger different rules. The load of concurrent requests is balanced by different chain nodes. The average latency of each test group is computed and Figure \ref{fig:macro-latency} shows the results of these experiments.

% Since the amount of chain nodes could affect the time it costs to reach a consensus, we vary the amount of chain nodes from 4 to 10 with 1000 fixed concurrent execution rules representing commonly used rules of a user. Figure \ref{fig:macro-latency} shows the average latency of each test group.

% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.21]{figrues/r2th.pdf}
% % \captionsetup{justification=centering}
% \caption{System Throughput With Various Numbers of IoT Rules}
% \label{fig:r2th}
% \end{figure}











